Monomial ideals with minimal generalized Barile-Macchia resolutions

We identify several classes of monomial ideals that possess minimal generalized Barile-Macchia resolutions. These classes of ideals include generic monomial ideals, monomial ideals with linear quotients, and edge ideals of hypertrees. We also characterize connected unicyclic graphs whose edge ideals are bridge-friendly and, in particular, have minimal Barile-Macchia resolutions. Barile-Macchia and generalized Barile-Macchia resolutions are cellular resolutions and special types of Morse resolutions.

==> commands.tex <==
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\sbridge}{sb}
\DeclareMathOperator{\mingens}{Gens}
\DeclareMathOperator{\BF}{BF}
\DeclareMathOperator{\w}{w}
\DeclareMathOperator{\dist}{dist}

\newcommand{\E}{\mathcal{E}}
\renewcommand{\H}{\mathcal{H}}

\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\NN}{{\mathbb N}}

\newcommand{\card}[1]{{\left\lvert #1 \right\lvert}}

\newcommand{\Kfoursymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
    baseline=-0.3ex,
    thick,
    ]
    \def\x{2.5mm};
    \def\r{0.2mm};
    \draw (0,0) -- (\x, 0) -- (\x, \x) -- (0, \x) -- cycle;
    \draw (0, 0) -- (\x, \x);
    \draw (\x, 0) -- (0, \x);

    \draw[fill=black] (0,0) circle (\r);
    \draw[fill=black] (0,\x) circle (\r);
    \draw[fill=black] (\x,0) circle (\r);
    \draw[fill=black] (\x,\x) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\diamondsymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
    baseline=-0.3ex,
    thick,
    ]
    \def\x{2.5mm};
    \def\r{0.11mm};
    \draw (0,0) -- (\x, 0) -- (\x, \x) -- (0, \x) -- cycle;
    \draw (0, 0) -- (\x, \x);

    \draw[fill=black] (0,0) circle (\r);
    \draw[fill=black] (0,\x) circle (\r);
    \draw[fill=black] (\x,0) circle (\r);
    \draw[fill=black] (\x,\x) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\gemsymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-0.25ex
    ]
    \def\x{2.5mm};
    \def\r{0.11mm};
    \draw (0,0) -- (\x/2, \x) -- (\x, 0) -- (3*\x/2, \x) -- (2*\x, 0) -- cycle;
    \draw (\x/2, \x) -- (3*\x/2, \x);

    \draw[fill=black] (0,0) circle (\r);
    \draw[fill=black] (\x/2, \x) circle (\r);
    \draw[fill=black] (\x,0) circle (\r);
    \draw[fill=black] (3*\x/2, \x) circle (\r);
    \draw[fill=black] (2*\x, 0) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\kitesymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{2.5mm};
    \def\r{0.11mm};
    \draw (0,0) -- (\x/2, \x/2) -- (\x, 0) -- (\x/2, -\x/2) -- cycle;
    \draw (\x/2, \x/2) -- (\x/2, -\x/2);
    \draw (\x,0) -- (3*\x/2,0);

    \draw[fill=black] (0,0) circle (\r);
    \draw[fill=black] (\x/2, \x/2) circle (\r);
    \draw[fill=black] (\x,0) circle (\r);
    \draw[fill=black] (\x/2, -\x/2) circle (\r);
    \draw[fill=black] (3*\x/2,0) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\pawsymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{2.5mm};
    \def\r{0.11mm};
    \draw (\x/2, \x/2) -- (\x, 0) -- (\x/2, -\x/2) -- cycle;
    \draw (\x,0) -- (3*\x/2,0);

    \draw[fill=black] (\x/2, \x/2) circle (\r);
    \draw[fill=black] (\x, 0) circle (\r);
    \draw[fill=black] (\x/2, -\x/2) circle (\r);
    \draw[fill=black] (3*\x/2,0) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\tadpolesymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
				thick,
		baseline=-1ex
		]
		\def\x{3mm};
		\def\r{0.11mm};
		\draw (\x/2, \x/2) -- (\x, 0) -- (\x/2, -\x/2) -- cycle;
		\draw (\x,0) -- (3 * \x/2, 0) -- (4*\x/2, -\x/2);

        \draw[fill=black] (\x/2, \x/2) circle (\r);
        \draw[fill=black] (\x, 0) circle (\r);
        \draw[fill=black] (\x/2, -\x/2) circle (\r);
        \draw[fill=black] (3*\x/2,0) circle (\r);
        \draw[fill=black] (4*\x/2, -\x/2) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\butterflysymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{3mm};
    \def\r{0.11mm};
    \draw (\x/2, \x/2) -- (\x, 0) -- (\x/2, -\x/2) -- cycle;
    \draw (3*\x/2, \x/2) -- (\x, 0) -- (3*\x/2, -\x/2) -- cycle;
    \draw[fill=black] (\x/2, \x/2) circle (\r);
    \draw[fill=black] (\x, 0) circle (\r);
    \draw[fill=black] (\x/2, -\x/2) circle (\r);
    \draw[fill=black] (3*\x/2, \x/2) circle (\r);
    \draw[fill=black] (3*\x/2, -\x/2) circle (\r);
    \end{tikzpicture}%
}

\newcommand{\sunletsymb}[2][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{1mm};
    \def\r{0.11mm};
    \def\theta{360/#2};

    \foreach \i in {1,...,#2}{
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({\x*cos(\theta*(\i+1))}, {\x*sin(\theta*(\i+1))});
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)});
        
        \draw[fill=black] ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) circle (\r);
        \draw[fill=black] ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)}) circle (\r);
    }
    \end{tikzpicture}%
}

\newcommand{\sixcycleconsecutivesymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{1mm};
    \def\theta{60};
    \def\r{0.11mm};

    \foreach \i in {1,...,6}{
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({\x*cos(\theta*(\i+1))}, {\x*sin(\theta*(\i+1))});

        \draw[fill=black] ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) circle (\r);
    }
    \foreach \i in {-1,0,1}{
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)});

        \draw[fill=black] ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)}) circle (\r);
    }
    \end{tikzpicture}%
}

\newcommand{\sixcyclealternatesymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
        thick,
    baseline=-1ex
    ]
    \def\x{1mm};
    \def\theta{60};
    \def\r{0.1mm};

    \foreach \i in {1,...,6}{
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({\x*cos(\theta*(\i+1))}, {\x*sin(\theta*(\i+1))});

        \draw[fill=black] ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) circle (\r);
    }
    \foreach \i in {-1,1,3}{
        \draw ({\x*cos(\theta*\i)}, {\x*sin(\theta*\i)}) -- ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)});

        \draw[fill=black] ({2*\x*cos(\theta*\i)}, {2*\x*sin(\theta*\i)}) circle (\r);
    }
    \end{tikzpicture}%
}

\newcommand{\starsymb}[1][0.5]{%
    \begin{tikzpicture}[scale=#1, %
		baseline=-0.3ex,
		thick,
		]
		\def\x{10mm};
		\def\r{0.8mm};
		\def\del{1.8mm};
		\def\rdel{0.3mm};
		\draw (0,0) -- (\x, \x);
		\draw (0,0) -- (\x, -\x);
		\draw (0,0) -- (-\x, \x);
		\draw (0,0) -- (-\x, -\x);
		\draw[fill=black] (0,0) circle (\r);
		\draw[fill=black] (\x, \x) circle (\r);
		\draw[fill=black] (\x, -\x) circle (\r);
		\draw[fill=black] (-\x, \x) circle (\r);
		\draw[fill=black] (-\x, -\x) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\gapfreetreesymb}[1][0.5]{%
    \begin{tikzpicture}[scale=#1, %
		baseline=-0.3ex,
		thick,
		]
		\def\x{15mm};
		\def\r{0.8mm};
		
		\draw (0,0) -- (\x, 0);
		
		\draw (0,0) -- (-0.6 * \x, 0.8 * \x);
		\draw (0,0) -- (-\x, 0);
		\draw (0,0) -- (-0.6 * \x, -0.8 * \x);
		
		\draw (\x, 0) -- (\x + 0.6 * \x, 0.8 * \x);
		\draw (\x, 0) -- (\x + \x, 0);
		\draw (\x, 0) -- (\x + 0.6 * \x, -0.8 * \x);
		
		\draw[fill=black] (0,0) circle (\r);
		\draw[fill=black] (\x,0) circle (\r);
		
		\draw[fill=black] (-0.6 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (-\x, 0) circle (\r);
		\draw[fill=black] (-0.6 * \x, -0.8 * \x) circle (\r);
		
		\draw[fill=black] (\x + 0.6 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (\x + \x, 0) circle (\r);
		\draw[fill=black] (\x + 0.6 * \x, -0.8 * \x) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\gapfreetreetrianglesymb}[1][0.5]{%
    \begin{tikzpicture}[scale=#1, %
		baseline=-0.3ex,
		thick,
		]
		\def\x{15mm};
		\def\r{0.8mm};
		
		\draw (0,0) -- (\x, 0);
		
		\draw (0,0) -- (-0.6 * \x, 0.8 * \x);
		\draw (0,0) -- (-\x, 0);
		\draw (0,0) -- (-0.6 * \x, -0.8 * \x);
		
		\draw (\x, 0) -- (\x + 0.6 * \x, 0.8 * \x);
		\draw (\x, 0) -- (\x + \x, 0);
		\draw (\x, 0) -- (\x + 0.6 * \x, -0.8 * \x);
		
		\draw (0, 0) -- (0.5 * \x, 0.8 * \x) -- (\x, 0);
		\draw (0, 0) -- (0.5 * \x, -0.8 * \x) -- (\x, 0);
		\draw (0, 0) -- (0.5 * \x, 1.2 * \x) -- (\x, 0);
		
		\draw[fill=black] (0,0) circle (\r);
		\draw[fill=black] (\x,0) circle (\r);
		
		\draw[fill=black] (0.5 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (0.5 * \x, -0.8 * \x) circle (\r);
		\draw[fill=black] (0.5 * \x, 1.2 * \x) circle (\r);
		
		
		\draw[fill=black] (-0.6 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (-\x, 0) circle (\r);
		\draw[fill=black] (-0.6 * \x, -0.8 * \x) circle (\r);
		
		\draw[fill=black] (\x + 0.6 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (\x + \x, 0) circle (\r);
		\draw[fill=black] (\x + 0.6 * \x, -0.8 * \x) circle (\r);
	\end{tikzpicture}%
}
\newcommand{\trianglesymb}[1][0.5]{%
    \begin{tikzpicture}[scale=#1, %
		baseline=1ex,
		thick,
		]
		\def\x{15mm};
		\def\r{0.8mm};
		
		\draw (0, 0) -- (0.5 * \x, 0.8 * \x) -- (\x, 0) -- cycle;
		\draw[fill=black] (0, 0) circle (\r);
		\draw[fill=black] (0.5 * \x, 0.8 * \x) circle (\r);
		\draw[fill=black] (\x, 0) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\pathsymb}[2][0.5]{%
    \begin{tikzpicture}[scale=#1, %
				thick,
		baseline=-0.5ex
		]
		\def\x{15mm};
		\def\r{0.8mm};
		
		\draw[fill=black] (0, 0) circle (\r);
		
		\foreach \i in {1,...,{#2}}{
			\draw ({(\i - 1) * \x}, {0}) -- ({\i * \x}, {0});
			\draw[fill=black] ({\i * \x}, {0}) circle (\r);
		}
	\end{tikzpicture}%
}

\newcommand{\dotsymb}[1][1]{%
    \begin{tikzpicture}[scale=#1, %
				thick,
		baseline=-0.5ex
		]
		\def\x{15mm};
		\def\r{0.8mm};
		\draw[fill=black] (0, 0) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\smallestcounterexamplesymb}{%
	\begin{tikzpicture}[scale=0.8, inner sep=0pt, baseline=0ex]
		\def\x{7mm};
		\def\r{0.45mm};
		
	    \node (t) at (-2*\x, 0) {};
	    \node (u) at (0, \x) {};
	    \node (v) at (\x, 0) {};
	    \node (w) at (0, 0) {};
	    \node (x) at (-\x, 0) {};
	    \node (y) at (0, -\x) {};
	    \node (z) at (2*\x, 0) {};

	    \draw[] (t) to (x);
	    \draw[] (x) to (w);
	    \draw[] (u) to (v);
	    \draw[] (u) to (x);
	    \draw[] (v) to (w);
	    \draw[] (y) to (v);
	    \draw[] (y) to (x);
	    \draw[] (v) to (z);

	    \draw[fill=black] (t) circle (\r);
	    \draw[fill=black] (u) circle (\r);
	    \draw[fill=black] (v) circle (\r);
	    \draw[fill=black] (w) circle (\r);
	    \draw[fill=black] (x) circle (\r);
	    \draw[fill=black] (y) circle (\r);
	    \draw[fill=black] (z) circle (\r);
	\end{tikzpicture}%
}

\newcommand{\joinsixcyclessymb}{%
\begin{tikzpicture}[scale=0.8,every node/.style={draw=black,circle}]
		\def\x{15mm};
		\def\r{0.8mm};
		
		\node[] (s) at (0, 1.5*\x) {$s$};
        \node[] (t) at (-1*\x, 0.5*\x) {$t$};
        \node[] (u) at (0, 0.5*\x) {$u$};
        \node[] (v) at (1*\x, 0.5*\x) {$v$};
        \node[] (w) at (-1*\x, -0.5*\x) {$w$};
        \node[] (x) at (0, -0.5*\x) {$x$};
        \node[] (y) at (1*\x, -0.5*\x) {$y$};
        \node[] (z) at (0, -1.5*\x) {$z$};

        \draw[] (s) to (t);
        \draw[] (s) to (u);
        \draw[] (s) to (v);
        \draw[] (t) to (w);
        \draw[] (u) to (x);
        \draw[] (v) to (y);
        \draw[] (w) to (z);
        \draw[] (x) to (z);
        \draw[] (y) to (z);
	\end{tikzpicture}%
}

\newcommand{\nonrootedhypertreesymb}{%
\begin{tikzpicture}[scale=1, %
    		baseline=1ex,
    		thick,
            every node/.style={inner sep=0,outer sep=0}
    		]
    		\def\x{15mm};
    		\def\r{0.3mm};

            \node[label={[xshift=0.8em, yshift=0em] \small $v$}] (v) at (0, 0) {};
            \draw[fill=black] (v) circle (\r);
            
            \foreach \theta/\vertex in {180/x, -60/y, 60/z} {
                \node[label={[xshift=0em, yshift=-1em] \small $\vertex$}] (\vertex) at ({\x * cos(\theta)}, {\x * sin(\theta)}) {};

                \node[label={[xshift=0em, yshift=-1em] \small $\vertex'$}] (\vertex\vertex) at ({2 * \x * cos(\theta)}, {2 * \x * sin(\theta)}) {};
            
                \draw (v) -- (\vertex);
                \draw (\vertex) -- (\vertex\vertex);

                \draw[fill=black] (\vertex) circle (\r);
                \draw[fill=black] (\vertex\vertex) circle (\r);
            };
	\end{tikzpicture}%
}

\newcommand{\cricketsymb}{%
\begin{tikzpicture}[scale=1, %
		baseline=1ex,
		thick,
		]
		\def\x{15mm};
		\def\r{0.3mm};

        \node[label={[xshift=-0.8em, yshift=-1em] \small $x$}] (x) at (0, 0) {};
        \node[label={[xshift=0.8em, yshift=-1em] \small $y$}] (y) at (\x, 0) {};
        \node[label={[xshift=-0.8em, yshift=-1em] \small $z$}] (z) at (0.5 * \x, 0.8 * \x) {};

        \node[label={[xshift=0em, yshift=-1.3em] \small $\cdots$}] (dots) at (0.5 * \x, 0.8 * \x + 0.5 * \x) {};
  
		\draw (0, 0) -- (0.5 * \x, 0.8 * \x) -- (\x, 0) -- cycle;

        \foreach \i in {-1, 1}{
            \foreach \j in {0.5, 0.7}{
                 \draw (0.5 * \x, 0.8 * \x) -- (0.5 * \x + \i * \j * \x, 0.8 * \x + 0.5 * \x);
                 \draw[fill=black] (0.5 * \x + \i * \j * \x, 0.8 * \x + 0.5 * \x) circle (\r);
            }
        }
  
		\draw[fill=black] (x) circle (\r);
		\draw[fill=black] (y) circle (\r);
		\draw[fill=black] (z) circle (\r);
	\end{tikzpicture}%
}
